Stochastic Multi-armed Bandits with Non-stationary Rewards Generated by a Linear Dynamical System

The stochastic multi-armed bandit has provided a framework for studying decision-making in unknown environments. We propose a variant of the stochastic multi-armed bandit where the rewards are sampled from a stochastic linear dynamical system. The proposed strategy for this stochastic multi-armed bandit variant is to learn a model of the dynamical system while choosing the optimal action based on the learned model. Motivated by mathematical finance areas such as Intertemporal Capital Asset Pricing Model proposed by Merton and Stochastic Portfolio Theory proposed by Fernholz that both model asset returns with stochastic differential equations, this strategy is applied to quantitative finance as a high-frequency trading strategy, where the goal is to maximize returns within a time period.

==> notes.tex <==
% \begin{theorem}\label{theorem:martingale_bound}
%     Let $\mathcal{F}_t$ be a filtration. Let $\Theta_{t;s}\in \mathbb{R}^{ms+1}$ and $\varepsilon_{A;t} \in \mathbb{R}$ be stochastic processes such that $\Theta_{t;s}$, $\varepsilon_{A;t}$ are $\mathcal{F}_t$ measurable and $\varepsilon_{A;t} \triangleq C_{A}(z_t - \hat{z}_t) + \eta_t $ is $\mathcal{F}_{t-1}$-conditionally $C_{A}PC_{A}^\top + R_{\eta}$-sub-Gaussian. Let there be the matrix defined in equation \eqref{eq:identify_V} and the matrix below:
%     \begin{equation}
%         \mathcal{S}_{N_{A};A,s} = \sum_{\tau \in \mathcal{T}_a} \varepsilon_{A;\tau} \Theta_{\tau;s}^{\top} . \label{eq:model_error_matrix_3}
%     \end{equation}
    
%     For any $\delta > 0$, with a probability of at least $1 - \delta$ for all $N_{A} \geq 0$: 
%     \begin{multline}\label{eq:martingale_bound}
%         ||\mathcal{S}_{N_{A};A,s}||_{V_{s}(N_{A})^{-1}}^2 \leq 4(C_{A}PC_{A}^\top + R_{\eta}) 
%         \Big(\log\big(1/\delta\big) \\ + \log\big(\det(V_{s}(N_{A}))/\det(\lambda I_{ms+1 }) + 1\big)\Big),
%     \end{multline}
%     where $||\mathcal{S}_{N_{A};A,s}||_{V_{s}(N_{A})^{-1}}^2$ is defined to be to 
%     \begin{equation}
%         ||\mathcal{S}_{N_{A};A,s}||_{V_{s}(N_{A})^{-1}}^2 \triangleq \mbox{Tr}(\mathcal{S}_{N_{A};A,s} V_{s}(N_{A})^{-1}\mathcal{S}_{N_{A};A,s}^\top).
%     \end{equation}
% \end{theorem}

% \begin{lemma}\label{lemma:bias_term}
%     Let linear system \eqref{eq:Linear_System} be converted to the following form 
%     \begin{equation}\label{eq:Kalman_System}
%         \begin{array}{ll}
%             \hat{z}_{t+1} & = (\Gamma -\Gamma KC_\theta)\hat{z}_t + K \theta_t  \\
%             X_t & = C_{A} \hat{z}_t + \varepsilon_{A;t}
%         \end{array}. 
%     \end{equation}
%     where $\varepsilon_{A;t} \triangleq C_A(z_t - \hat{z}_t) + \eta_t \sim \mathcal{N}(0,C_APC_A^\top + R_\eta)$. Therefore, equation \eqref{eq:Matrix_Form} can be expressed the following way
%     \begin{equation}
%         X_{t} = C_{A}(\Gamma-\Gamma K C_\theta)^s \hat{z}_{t-s} + G_{s}(A)\Theta_{t;s} + \varepsilon_{A;t}. 
%     \end{equation}
    
%     For the bias term $C_{A}(\Gamma-\Gamma K C_\theta)^s \hat{z}_{t-s}$ in equation \eqref{eq:Matrix_Form}, given a failure probability of $\delta \in (0,1)$, the following inequality is satisfied with a probability of at least $1-\delta$:
%     \begin{multline}
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2 \leq \\ B_1 ||V_s(N_A)^{-1}||_2 \Big(ms + \log(1/\delta) \\ + \log(\det(V_s(N_A))/\det(\lambda I_{ms+1}))\Big) + B_3,
%     \end{multline}
%     where $B_1$ and $B_3$ are defined to be 
%     \begin{align}
%         B_1 & \triangleq 2 ||C_{A}(\Gamma -\Gamma K C_\theta)^s ||_2^2 ||O(C_\theta,\Gamma,s)^\dagger||_2^2 \cdot \nonumber \\
%         & \quad\quad\quad\quad\quad\quad\quad\quad ||\Phi_{\theta}||_2^2 ||C_{\theta} P C_{\theta}^\top + R_{\phi}||_2^2 , \\
%         B_3 & \triangleq ||C_{A}(\Gamma -\Gamma K C_\theta)^s ||_2^2||O(C_\theta,\Gamma,s)^\dagger||_2^2,
%     \end{align}
%     and $O(C_{\theta},\Gamma,s)$ and $\Phi_{\theta}$ are the following matrices:
%     \begin{align}
%         O(C_{\theta},\Gamma,s) & \triangleq \begin{bmatrix}
%             C_{\theta}^\top & \dots & (\Gamma^\top)^s C_{\theta}^\top 
%         \end{bmatrix}^\top, \label{eq:Obs}\\
%         \Phi_{\theta} & \triangleq \begin{bmatrix}
%             I_{m} & \dots & 0 \\
%             \vdots & \ddots & \vdots \\
%             C_{\theta} \Gamma^{s-1} K & \dots & I
%         \end{bmatrix}. \label{eq:error_matrix}
%     \end{align}
% \end{lemma}
% \begin{proof}
%     For the bias term in equation \eqref{eq:Matrix_Form}, note the following inequality using the Cauchy Schwarz inequality
%     \begin{multline}
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2 \leq \\ ||C_{A}(\Gamma -\Gamma K C_\theta)^s||_2^2
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \hat{z}_{t-s}\Theta_{t;s}^\top \Bigg|\Bigg|_{V_s(N_A)^{-2}}^2.
%     \end{multline}
    
%     The vector $\Theta_{t;s}$ has the following expression:
%     \begin{align}
%         \Theta_{t;s} & = O(C_\theta,\Gamma,s) \hat{z}_{t-s} + \Phi_{\theta} E_{\theta}, \nonumber \\
%         \Rightarrow \hat{z}_{t-s}\Theta_{t;s}^\top & = O(C_\theta,\Gamma,s)^\dagger \Big(\Theta_{t;s}\Theta_{t;s}^\top - \Phi_{\theta} E_{\theta} \Theta_{t;s}^\top \Big),\nonumber
%     \end{align}
%     where $O(C_{\theta},\Gamma,s)$ is defined in equation \eqref{eq:Obs}, $\Phi_{\theta}$ is defined in equation \eqref{eq:error_matrix}, and $E_{\theta}$ is defined to be
%     \begin{equation}
%         E_{\theta} \triangleq \begin{bmatrix}
%             \varepsilon_{\theta;t-s} \\
%             \vdots \\
%             \varepsilon_{\theta;t-1}
%         \end{bmatrix} \in \mathbb{R}^{ms}.
%     \end{equation}
    
%     This leads to the following inequality
%     \begin{multline}
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \hat{z}_{\tau-s}\Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_s(N_A)^{-2}}^2 \leq \\
%         ||O(C_\theta,\Gamma,s)^\dagger||_2^2\Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}}\Theta_{t;s}\Theta_{t;s}^\top\Bigg|\Bigg|_{V_s(N_A)^{-2}}^2 \\ + ||O(C_\theta,\Gamma,s)^\dagger||_2^2\Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \Phi_{\theta} E_{\theta} \Theta_{t;s}^\top\Bigg|\Bigg|_{V_s(N_A)^{-2}}^2.\nonumber
%     \end{multline}
    
%     The first term has the following bound
%     \begin{multline}
%       ||O(C_\theta,\Gamma,s)^\dagger||_2^2\Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}}\Theta_{t;s}\Theta_{t;s}^\top\Bigg|\Bigg|_{V_s(N_A)^{-2}}^2\leq \\ ||O(C_\theta,\Gamma,s)^\dagger||_2^2.\nonumber
%     \end{multline}

%     Based on theorem 2 in \cite{sarkar2020nonparametric}, since $\Phi_\theta E_\theta$ is conditionally $||\Phi_{\theta}||_2^2 ||C_{\theta} P C_{\theta}^\top + R_{\phi}||_2^2$-sub-Gaussian and $\Theta_{t;s}$ is measurable, then given a failure probability of $\delta \in (0,1)$, the following inequality is satisfied with a probability at least $1-\delta$:
%     \begin{multline}
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \Phi_{\theta} E_{\theta} \Theta_{t;s}^\top\Bigg|\Bigg|_{V_s(N_A)^{-1}}^2 \leq 2 ||\Phi_{\theta}||_2^2 ||C_{\theta} P C_{\theta}^\top + R_{\phi}||_2^2 \cdot \\
%         \Big(ms + \log(1/\delta)  + \log(\det(V_s(N_A))/\det(I_{ms+1}))\Big). \nonumber
%     \end{multline}
    
%     Therefore, the following inequality is satisfied with a probability of $1-\delta$, $\delta \in (0,1)$ as the failure rate: 
%      \begin{multline}
%         \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2 \leq \\ B_1 ||V_s(N_A)^{-1}||_2 \Big(ms + \log(1/\delta) \\ + \log(\det(V_s(N_A))/\det(\lambda I_{ms+1}))\Big) + B_3.
%     \end{multline}
% \end{proof}

% \begin{theorem}\label{theorem:model_error}
%     Given that $\hat{G}_{s}(N_{A})$ is identified using equation \eqref{eq:identify}, with a failure probability of $\delta \in (0,1)$, the following inequality is satisfied with a probability of at least $1-\delta$:
%     \begin{equation}
%         ||\hat{G}_{s}(N_{A}) - G_{s}(A)||_2^2 \leq M(N_A),
%     \end{equation}
%     where $M(N_A)$ is defined to be
%     \begin{multline}\label{eq:M_Bound}
%         M(N_A) \triangleq  (B_1+B_2)||V_s(N_A)^{-1}||_2\Big(\log(1/\delta) \\ + \log(\det(V_{s}(N_{A}))/\det(\lambda I_{ms+1})) \Big) \\
%         + ||V_s(N_A)^{-1}||_2(ms B_1 + B_2) + B_3 \\ + \lambda^2 ||G_{s}(A)||_{V_{s}(N_{A})^{-2}}^2, 
%     \end{multline}
%     and $B_2$ is defined to be 
%     \begin{equation}
%         B_2 \triangleq (C_{A} P C_{A}^\top + R_\eta)^2.
%     \end{equation}
% \end{theorem}
% \begin{proof}
%     % Let linear system \eqref{eq:Linear_System} be converted to the following form 
%     % \begin{equation}
%     %     \begin{array}{ll}
%     %         \hat{z}_{t+1} & = (\Gamma -\Gamma KC_\theta)\hat{z}_t + K \theta_t  \\
%     %         X_t & = C_{A} \hat{z}_t + \varepsilon_{A;t}
%     %     \end{array}. 
%     % \end{equation}
%     % where $\varepsilon_{A;t} \triangleq C_A(z_t - \hat{z}_t) + \eta_t \sim \mathcal{N}(0,C_APC_A^\top + R_\eta)$. Therefore, equation \eqref{eq:Matrix_Form} can be expressed the following way
%     % \begin{equation}
%     %     X_{t} = C_{A}(\Gamma-\Gamma K C_\theta)^s \hat{z}_{t-s} + G_{s}(A)\Theta_{t;s} + \varepsilon_{A;t}. 
%     % \end{equation}
%     Using equation \eqref{eq:identify} and \eqref{eq:Kalman_System}, the difference $\hat{G}_{s}(N_{A}) - G_s(A)$ has the following expression

%     % \begin{align}
%     %     \hat{G}_{s}(N_{A}) & = \sum_{\tau \in \mathcal{T}_{A}} G_{s}(A)\Theta_{\tau;s} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\
%     %     &\quad\quad + C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\
%     %     & \quad\quad + \varepsilon_{A;\tau} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1}, \nonumber \\
%     %     & = G_{s}(A) (V_{s}(N_{A}) - \lambda I) V_{s}(N_{A})^{-1}   \nonumber\\ 
%     %     & \quad\quad + \sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\ 
%     %     & \quad\quad + \sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\ 
%     %     & \quad\quad + \lambda G_{s}(A) V_{s}(N_{A})^{-1} - \lambda G_{s}(A) V_{s}(N_{A})^{-1}, \nonumber 
%     % \end{align}
%     % \begin{align}
%     %     & = G_{s}(A) - \lambda G_{s}(A) V_{s}(N_{A})^{-1}\nonumber\\ 
%     %     & \quad\quad + \sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\ 
%     %     & \quad\quad + \sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1}, \nonumber 
%     % \end{align}
%     \begin{align}
%         \hat{G}_{s}(N_{A}) - G_{s}(A) & = - \lambda G_{s}(A) V_{s}(N_{A})^{-1}\nonumber\\ 
%         &+ \sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1} \nonumber \\ 
%         &+ \sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top V_{s}(N_{A})^{-1},     \nonumber
%     \end{align}
    
%     Using the triangle inequality and Cauchy Schwarz inequality, the $\ell$-2 norm $||\hat{G}_{s}(N_{A}) - G_{s}(A)||_2^2$ has the following upper bound:
%     % \begin{multline}
%     %     ||\hat{G}_{s}(N_{A}) - G_{s}(A)||_2^2 \leq \lambda^2 ||G_{s}(A)||_{V_{s}(N_{A})^{-2}}^2 \\ 
%     %     + \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2 \\ 
%     %     + \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top\Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2. 
%     % \end{multline}
%     \begin{multline}
%         ||\hat{G}_{s}(N_{A}) - G_{s}(A)||_2^2 \leq \lambda^2 ||G_{s}(A)||_{V_{s}(N_{A})^{-2}}^2 \\ 
%         + \Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} C_{A}(\Gamma -\Gamma K C_\theta)^s \hat{z}_{\tau-s} \Theta_{\tau;s}^\top \Bigg|\Bigg|_{V_{s}(N_{A})^{-2}}^2 \\ 
%         + ||V_s(N_A)^{-1}||_2\Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top\Bigg|\Bigg|_{V_{s}(N_{A})^{-1}}^2. \nonumber
%     \end{multline}
    
%     The variable $\varepsilon_{A;t}$ is $C_{A} P C_{A}^\top + R_\eta$-Gaussian distributed and $\Theta_{t;s}$ is measurable. Therefore, based on theorem 2 in \cite{sarkar2020nonparametric}, given a failure rate of $\delta \in (0,1)$, the following inequality is satisfied with a probability of at least $1-\delta$
%     \begin{multline}\label{eq:cross_term_error}
%         ||V_s(N_A)^{-1}||_2\Bigg|\Bigg|\sum_{\tau \in \mathcal{T}_{A}} \varepsilon_{A;\tau} \Theta_{\tau;s}^\top\Bigg|\Bigg|_{V_{s}(N_{A})^{-1}}^2 \leq
%         \\ 2||V_s(N_A)^{-1}||_2(C_{A} P C_{A}^\top + R_\eta)^2 \cdot \\ \Big(\log(1/\delta)  + \log(\det(V_{s}(N_{A}))/\det(\lambda I_{ms+1})) + 1)\Big). \nonumber
%     \end{multline}
    
%     Using lemma \ref{lemma:bias_term} for the bias term, this gives the final inequality 
%     \begin{multline}
%         ||\hat{G}_{s}(N_{A}) - G_{s}(A)||_2^2 \leq (B_1+B_2)||V_s(N_A)^{-1}||_2\Big(\log(1/\delta) \\ + \log(\det(V_{s}(N_{A}))/\det(\lambda I_{ms+1})) \Big) \\
%         + ||V_s(N_A)^{-1}||_2(ms B_1 + B_2) + B_3 \\ +  \lambda^2 ||G_{s}(A)||_{V_{s}(N_{A})^{-2}}^2. 
%     \end{multline}
% \end{proof}

\begin{lemma}\label{lemma:E_1}
    Given the event $\mathcal{E}_1$ which is defined to be 
    \begin{equation}
        \mathcal{E}_1 \triangleq \{\tilde{G}_{s}(N_A) \Theta_{t;s} \geq C_{A^*}z_t\},
    \end{equation}
    if the number of times action $A$ has been chosen is 
    \begin{equation}\label{eq:u_a_set}
        u_{A} \triangleq \frac{B_3}{\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s} - \sigma^2/2},
    \end{equation}
    where $\sigma^2$ is defined to be 
    \begin{equation}\label{eq:sigma_bound}
        \sigma^2 \triangleq C_{A} (\Gamma - \Gamma K C_\theta)^s P ((\Gamma - \Gamma K C_\theta)^\top )^s C_{A}^\top + C_{A} P C_{A}^\top,
    \end{equation}
    then the probability of event $\mathcal{E}_1$ conditioned on $\mathcal{Z}_t$, where $\mathcal{Z}_t$ is the sigma algebra generated by states $z_0,\dots,z_t$, is at most $\delta$. 
\end{lemma}
    
\begin{proof}
    For event $\mathcal{E}_1$, the inequality is as follows 
    \begin{align}
        \tilde{G}_{s}(N_A) \Theta_{t;s} & \geq C_{A^*}z_t, \nonumber \\
        \tilde{G}_{s}(N_A) \Theta_{t;s} - C_{A} z_t & \geq C_{A^*}z_t - C_{A} z_t, \nonumber \\
        \tilde{G}_{s}(N_A) \Theta_{t;s} - G_{s}(A) \Theta_{t;s} \nonumber \\
        - C_{A} (\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} \nonumber \\
        - \gamma_{A;t} & \geq \Delta C_{A} z_t, \nonumber \\
        ||\tilde{G}_{s}(N_A) - G_{s}(A) ||_{\Theta_{t;s}\Theta_{t;s}^\top} 
        & \geq \Delta C_{A} z_t \nonumber \\
        & \quad + C_{A} (\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} \nonumber \\
        & \quad +  \gamma_{A;t}, \nonumber 
    \end{align}    
    where $\gamma_{A;t} \triangleq C_A(z_t - \hat{z}_t) \sim \mathcal{N}(0,C_APC_A^\top)$. Set $u_A \geq 0$ to be a variable free to be chosen. This adjusts the inequality to be the following
    \begin{align}
        \frac{1}{u_{A}}||\tilde{G}_{s}(N_A) - G_{s}(A) ||_{u_A I_{ms+1}+ \Theta_{t;s}\Theta_{t;s}^\top} 
        & \geq \Delta C_{A} z_t \nonumber \\
        & \quad + C_{A} (\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} \nonumber \\
        & \quad +  \gamma_{A;t}. \nonumber
    \end{align}
    
    Based on theorem \ref{theorem:model_error}, given a failure rate of $\delta \in (0,1)$, the following inequality is satisfied with a probability of at least $1-\delta$: 
    \begin{equation}\label{eq:inequality_6}
        ||\hat{G}_{s}(N_A) - G_{s}(A) ||_2 \leq M(N_A). \nonumber
    \end{equation}
    
    Therefore, the following inequality is satisfied with a probability of at most $\delta$:
    \begin{align}\label{eq:inequality_7}
        ||\tilde{G}_{s}(N_A) - G_{s}(A) ||_{u_A I_{ms+1}+ \Theta_{t;s}\Theta_{t;s}^\top } & > ||\hat{G}_{s}(N_A) - G_{s}(A) ||_2 , \nonumber \\
        & > M(N_A). \nonumber
    \end{align}
    
    Note $M(N_A)$ is lower bounded by the following inequality:
    \begin{equation}
        M(N_A) \geq B_3. \nonumber
    \end{equation}
    
    This leads to the inequality below which is satisfied with a probability of at most $\delta$
    \begin{equation}\label{eq:inequality_8}
        \frac{1}{u_{A}}||\tilde{G}_{s}(N_A) - G_{s}(A) ||_{u_A I_{ms+1}+ \Theta_{t;s}\Theta_{t;s}^\top } > \frac{B_3}{u_{A}} .\nonumber
    \end{equation}
    
    Since $u_A$ is free to be chosen, we set $u_A$ such that the following inequality is satisfied:
    \begin{equation}
         \frac{B_3}{u_{A}} \geq \Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} +  \gamma_{A;t}.\nonumber
    \end{equation}

    The random variable on the right-hand-side is a Gaussian distribution. Therefore, by symmetry of Gaussian distributions, the inequality can be adjusted to be 
    \begin{equation}
        - \Delta C_{A} z_t - C_{A} (\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} -  \gamma_{A;t} \geq \frac{-B_3}{u_{A}}.\nonumber
    \end{equation}
    
    The random variable on the left-hand-side of the equation has a constant conditional mean and variance, where the conditional variance is bounded by equation \eqref{eq:sigma_bound}. This leads to the following concentration bound using the Markov inequality and the moment generating function for normal distributions, where for $\alpha > 0$
    \begin{multline}
        \mathbb{P}[\mathcal{E}_1|\mathcal{Z}_t] \leq \delta \exp\Big\{- \alpha(\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s})\\ + \frac{B_3}{u_{A}} + \frac{\alpha^2 \sigma^2}{2} \Big\}.\nonumber
    \end{multline}

    Setting $\alpha = 1$ gives the following 
    \begin{multline}
        \mathbb{P}[\mathcal{E}_1|\mathcal{Z}_t] \leq \delta \exp\Big\{- (\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s}) \\ + \frac{B_3}{u_{A}} + \frac{\sigma^2}{2} \Big\}.\nonumber
    \end{multline}
    
    If $u_{A}$ is set such that  
    \begin{equation}
        u_{A} \triangleq \frac{B_3}{\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s} - \sigma^2/2},
    \end{equation}
    then the probability $\mathbb{P}[\mathcal{E}_1|\mathcal{Z}_t]$ occurs is at most $\delta$. 
    
\end{proof}

\begin{lemma}\label{lemma:E_2}
    Given the event $\mathcal{E}_2$ which is defined to be 
    \begin{equation}
        \mathcal{E}_2 \triangleq \{\tilde{G}_{s}(N_{A^*})\Theta_{t;s} \leq C_{A^*} z_t\},
    \end{equation}
    the probability of this event is upper-bounded by 
    \begin{multline}\label{eq:E_2_bound}
        \mathbb{P}[\mathcal{E}_2|\mathcal{Z}_t] \leq \frac{ \delta\Big(||C_{A^*}(\Gamma - \Gamma K C_\theta)^s z_{t-s}||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])} \\ + \frac{ \delta\Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s e_{t-s}||_2] + ||C_A P C_A^\top||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}.
    \end{multline}
\end{lemma}

\begin{proof}
    For the event $\mathcal{E}_2$, note the following 
    \begin{align}
        \tilde{G}_{s}(N_{A^*})\Theta_{t;s} & \leq C_{A^*} z_t, \nonumber \\
        (\tilde{G}_{s}(N_{A^*}) - G_{s}(A^*))\Theta_{t;s} & \leq C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s} + \gamma_{A^*;t}, \nonumber \\
        ||\tilde{G}_{s}(N_{A^*}) - G_{s}(A^*)||_{\Theta_{t;s}\Theta_{t;s}^\top} & \leq ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 \nonumber\\
        & \quad + ||\gamma_{A^*;t}||_2. \label{eq:inequality_3}
    \end{align}
    
    Note the following Markov inequality which is true with a probability of at most $1$:
    \begin{multline}
        \Theta_{t;s}\Theta_{t;s}^\top \geq \mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top],  \\
        \Rightarrow \sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])||\hat{G}_{s}(N_{A^*}) - G_{s}(A^*)||_2 \leq \\ ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2. 
    \end{multline}
    
    Given a failure probability of $\delta \in (0,1)$, the following inequality is satisfied with a probability of at most $\delta$. 
    \begin{equation}\label{eq:inequality_9}
        ||\tilde{G}_{s}(N_{A^*}) - G_{s}(A^*)||_2 \geq M(N_{A^*}).
    \end{equation}
    
    This updates inequality \eqref{eq:inequality_3} to the following 
    \begin{align}
        M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top]) & \leq
        ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 \nonumber \\
        & \quad + ||\gamma_{A^*;t}||_2. \nonumber
    \end{align}

    Therefore, using the inequalities mentioned above and by the Markov inequality, the following concentration bound is derived:
    \begin{multline}
        \mathbb{P} \Bigg[
        \nu  \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2|\mathcal{Z}_{t}]\Big) \\ \leq ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2
        \Bigg] \leq \frac{1}{\nu}.\nonumber
    \end{multline}
    
    Setting $\nu$ to the following
    \begin{equation}
        \nu = \frac{M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}{\Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2|\mathcal{Z}_{t}]\Big)},\nonumber
    \end{equation}
    then by equation \eqref{eq:inequality_9}, the following is true 
    \begin{multline}
        \mathbb{P} \Bigg[ M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top]) \leq  ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2  \\ + ||\gamma_{A^*;t}||_2
        \Bigg] \\ \leq  \frac{\delta \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2|\mathcal{Z}_{t}]\Big)}{M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}.\nonumber
    \end{multline}
    
    For $M(N_{A^*})$, this is lower bounded by the following
    \begin{align}
        M(N_{A^*}) & \geq B_3, \nonumber \\
        \frac{1}{M(N_{A^*})} & \leq \frac{1}{B_3}.\nonumber
    \end{align}
    
    With a failure rate of $\delta \in (0,1)$, this gives the following concentration inequality 
    \begin{multline}\label{eq:inequality_10}
        \mathbb{P} \Bigg[ M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])  \leq  ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2  \\ + ||\gamma_{A^*;t}||_2
        \Bigg] \\ \leq \frac{ \delta \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2 + ||\gamma_{A^*;t}||_2|\mathcal{Z}_{t}]\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}.
    \end{multline}
    
    Note that $e_{t-s} \triangleq z_{t-s} - \hat{z}_{t-s} \sim \mathcal{N}(0,P)$; therefore, inequality \eqref{eq:inequality_10} is updated to the following
    \begin{multline}
        \mathbb{P} \Bigg[ M(N_{A^*})\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top]) \leq  ||C_{A^*}(\Gamma - \Gamma K C_\theta)^s \hat{z}_{t-s}||_2  \\ + ||\gamma_{A^*;t}||_2
        \Bigg] \\ \leq \frac{ \delta \Big(||C_{A^*}(\Gamma - \Gamma K C_\theta)^s z_{t-s}||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])} \\ + \frac{ \delta \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s e_{t-s}||_2] + ||C_A P C_A^\top||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}.\nonumber
    \end{multline}
\end{proof}

Lemmas \ref{lemma:E_1} and \ref{lemma:E_2} prove the upper bound for the probability of two events where algorithm \ref{alg:cap} chooses an action that does not return the highest reward at a given round $t$ conditioned on $\mathcal{Z}_t$. Using these lemmas, the regret can be proven in the following theorem. 

\begin{theorem}\label{theorem:regret}
    Using algorithm \ref{alg:cap}, the upper bound for regret conditioned on $\mathcal{Z}_t$ is 
    \begin{multline}
         \sum_{t=1}^n \mathbb{E}[(C_{A^*} - C_A) z_t|\mathcal{Z}_t] \leq \\
         \sum_{t = 1}^n \Bigg(\frac{B_3}{\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s}-\sigma^2/2} + \delta \\ + \frac{ \delta \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s e_{t-s}||_2] + ||C_A P C_A^\top + R_\eta||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])} \\ + 
         \frac{ \delta\Big(||C_{A^*}(\Gamma - \Gamma K C_\theta)^s z_{t-s}||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}\Bigg) ||\Delta C_{A}z_t||_2.
    \end{multline}
    
    Under the case when $\rho(\Gamma) < 1$, regret increases at a rate of $\mathcal{O}(n)$. As for the case when $\rho(\Gamma) = 1$, regret increases at a rate of $\mathcal{O}(n^2)$. 
\end{theorem}
\begin{proof}
    Regret conditioned on $\mathcal{Z}_t$ is 
    \begin{align}
        R_n & = \sum_{t = 1}^n \mathbb{E}[C_{A^*} z_t - C_{A} z_t|\mathcal{Z}_{t}], \nonumber \\ 
        & = \sum_{t = 1}^n \mathbb{E}[\Delta C_{A} z_t|\mathcal{Z}_{t}] . \nonumber
    \end{align}
    For one arm $A \in \mathcal{A}$ at round $t = 1,\dots,n$, the expected regret of that arm at that round is the following
    \begin{align}
        \mathbb{E}[\Delta C_{A} z_t \mathbb{I}\{A = a\}|\mathcal{Z}_{t}] & = \mathbb{E}[\Delta C_{A} z_t \mathbb{I}\{\mathcal{E}_{A^*}\}|\mathcal{Z}_{t}] \nonumber \\
        & \quad + \mathbb{E}[\Delta C_{A} z_t \mathbb{I}\{\mathcal{E}_{A}\}|\mathcal{Z}_{t}], \nonumber \\
        & \leq \frac{u_{A}}{n}\mathbb{E}[\Delta C_{A} z_t|\mathcal{Z}_{t}] \nonumber \\
        & \quad + \mathbb{E}[\Delta C_{A} z_t|\mathcal{Z}_{t}]\mathbb{P}[\mathcal{E}_{A}|\mathcal{Z}_{t}].\nonumber
    \end{align}
    
    Therefore, the fixed value $u_{A}$ must be found. To find $u_{A}$, $u_{A}$ is based on the events $\mathcal{E}_{A^*}$ and $\mathcal{E}_{A}$ 
    \begin{align}
        \mathcal{E}_{A^*} & \triangleq \{\tilde{G}_{s}(N_A) \Theta_{t;s} < C_{A^*}z_t\} \cap \{\tilde{G}_{s}(N_{A^*})\Theta_{t;s} > C_{A^*} z_t\}, \nonumber \\
        \mathcal{E}_{A} & \triangleq \mathcal{E}_1 \cup \mathcal{E}_2 . \nonumber
    \end{align}
    
    For the good event $\mathcal{E}_{A^*}$, first assume that $u_{A}/n > \mathbb{I}\{\mathcal{E}_{A^*}\}$. This implies that by round $n$, there exists a round $t$ such that arm $A$ has been chosen $u_{A}$ times. However, by definition of $\mathcal{E}_{A^*}$, this implies
    \begin{equation}
        \tilde{G}_{s}(N_A) \Theta_{t;s} < C_{A^*} z_t < \tilde{G}_{s}(N_{A^*})\Theta_{t;s}. \nonumber
    \end{equation}

    Therefore, action $A^*$ is chosen, which is a contradiction as action $A$ must have been chosen more than $u_{A}$ times. This implies that $N_{A} \leq u_{A}$.     
    
    Now for the first event $\mathcal{E}_1$ of $\mathcal{E}_{A}$, using lemma \ref{lemma:E_1}, the probability of $\mathcal{E}_1$ occurs at most $\delta$ given that $u_{A}$ is set to equation \eqref{eq:u_a_set}. For the event $\mathcal{E}_2$, based on lemma \ref{lemma:E_2}, the probability of event $\mathcal{E}_2$ is upper-bounded by \eqref{eq:E_2_bound}. This gives the final inequality for total regret
    \begin{multline}
        \sum_{t = 1}^n \mathbb{E}[\Delta C_{A} z_t|\mathcal{Z}_t] \leq \\
         \sum_{t = 1}^n \Bigg(\frac{B_3}{\Delta C_{A} z_t + C_{A} (\Gamma - \Gamma K C_\theta)^s z_{t-s}-\sigma^2/2} + \delta + \\ + \frac{ \delta \Big(\mathbb{E}[||C_{A^*}(\Gamma - \Gamma K C_\theta)^s e_{t-s}||_2] + ||C_A P C_A^\top + R_\eta||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}\\ + \frac{ \delta \Big(||C_{A^*}(\Gamma - \Gamma K C_\theta)^s z_{t-s}||_2\Big)}{B_3\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])}\Bigg) ||\Delta C_{A}z_t||_2.
    \end{multline}
    
    The dominating terms in the summation above are the terms $z_{t-s}$ and $z_t$. If $\rho(\Gamma) < 1$, then all the terms in the summation are constant, implying regret grows at a rate of $\mathcal{O}(n)$. If $\rho(\Gamma) = 1$, then $||z_t||_2$ grows at a rate of $t\mbox{Tr}(Q)$. However, $\sigma_{\min}(\mathbb{E}[\Theta_{t;s}\Theta_{t;s}^\top])$ also grows at a rate $t \sigma_{\min}(C_\theta Q C_\theta + R_\phi/t)$. This leads to a partial summation of $t$ terms, which is $\mathcal{O}(n^2)$. Therefore, total regret is $\mathcal{O}(n^2)$. 
    
\end{proof}



% Variants have been proposed for the multi-armed bandit to focus on the cases when the learner may interact with a dynamic environment. For example, the adversarial multi-armed bandit focuses on when the distribution of the rewards can be changed by an adversary at any given time \cite{auer2002nonstochastic}. Other results have observed the case when the reward distributions stochastically change. When the rewards follows a known stochastic transition function is called the \textit{restless bandit} \cite{whittle1988restless}. If the stochastic process is unknown, the non-stationary bandit problem is introduced, where the distribution of the reward in an environment changes over time. Results for the non-stationary bandit problem are an UCB based method for the problem \cite{garivier2008upper}, applying reinforcement learning methods \cite{koulouriotis2008reinforcement}, a Bayesian approach \cite{raj2017taming}, and exploring arms at a rate for efficient learning \cite{gafni2020learning}. Other papers have focused on how the distributions in the non-stationary bandit problem change such as the distribution can only change a set number of times \cite{besbes2014stochastic} or the mean of the distribution follows a Brownian motion process or random walk \cite{slivkins2008adapting}.


